Characterization of the errors of the FMM in particle simulations

The Fast Multipole Method (FMM) offers an acceleration for pairwise interaction calculation, known as $N$-body problems, from $\mathcal{O}(N^2)$ to $\mathcal{O}(N)$ with $N$ particles. This has brought dramatic increase in the capability of particle simulations in many application areas, such as electrostatics, particle formulations of fluid mechanics, and others. Although the literature on the subject provides theoretical error bounds for the FMM approximation, there are not many reports of the measured errors in a suite of computational experiments. We have performed such an experimental investigation, and summarized the results of about 1000 calculations using the FMM algorithm, to characterize the accuracy of the method in relation with the different parameters available to the user. In addition to the more standard diagnostic of the maximum error, we supply illustrations of the spatial distribution of the errors, which offers visual evidence of all the contributing factors to the overall approximation accuracy: multipole expansion, local expansion, hierarchical spatial decomposition (interaction lists, local domain, far domain). This presentation is a contribution to any researcher wishing to incorporate the FMM acceleration to their application code, as it aids in understanding where accuracy is gained or compromised.

==> intro.tex <==
%%  INTRODUCTION


In particle simulations, often the dynamics results from the summation of all pair-wise forces in the ensemble of particles.  Such situations arise in astrophysics, molecular dynamics, plasma physics, and certain formulations of fluid dynamics problems, for example.  The total field of interest (gravitational, electrostatic, etc.) at one evaluation point requires adding the contribution of all source points or particles, and so if both evaluation points and particles are numbered at $N$, a total of $N^2$ operations is needed.  This fact was for a long time an impediment to the wider use of particle simulations, as the computational effort becomes prohibitive for large numbers of particles.

The above scenario changed dramatically with the introduction of tree-codes and the fast multipole method (FMM), which appear in the late 1980s for accelerated evaluation of $N$-body problems.  Tree-codes \cite{Appel1985,BarnesHut1986} are generally perceived to be easier to grasp and program, and provide a complexity of $\mathcal{O}(N \log N)$.  The FMM was introduced as an algorithm for the rapid evaluation of gravitational or Coulombic interactions \cite{greengard+rokhlin1987} and promises a reduction in computational complexity to $\mathcal{O}(N)$.  It has, since its dissemination, been adapted for many applications:  for fast evaluation of boundary elements \cite{Gaspar1998}, for vortex sheet problems with desingularized equations \cite{HamiltonMajda1995}, for long-range electrostatics in DNA simulations \cite{FenleyETal1996}, and many others.  The impact of the FMM has been undeniably huge, resulting in it being chosen as one of the Top 10 Algorithms of the 20th Century \cite{DongarraSulli2000}.

Despite the great volume of work using and adapting the FMM in many application areas, there remains some lack of insight regarding how the algorithm can be efficiently used to obtain an accurate representation of the field of interest.  The error of the FMM approximation is estimated by theoretical bounds, which as could be expected reveal a trade-off between accuracy and efficiency of the computation.  However, there is not much literature providing measurements of the accuracy of the approximation, in practice.  One may often find such assertions in published works as ``only the first three moments of the expansion were used'', or something to that effect.  But just as often there is no information provided about the actual errors which are \emph{observed}.  Of course, it is not easy to provide such measures of observed error, as this would require additional computations using the direct $\mathcal{O}(N^2)$ method, for comparison purposes. Nevertheless, it is important for users of the algorithm to know what to expect in terms of accuracy and efficiency, depending on the choice of algorithm parameters.

We aim to contribute to this gap in understanding by presenting a methodical investigation into the errors of the approximation used by the FMM, when the underlying `client' application is the calculation of the velocity field induced by $N$ regularized particles of vorticity.  This application is rather more demanding than the Newtonian force calculation, because in the latter case the gravitational interaction is dominated by the first moment ---due to the fact that all mass is positive.  Therefore, keeping only the first three moments could easily give the desired accuracy.  On the other hand, as in Coulomb electrostatic calculations, the vortex particles can be both positive and negative, and thus an acceptable accuracy may require that more terms in the expansion be kept. 

For the purposes of this study, a prototype code of the FMM computation of the velocity induced by $N$ vortex particles was implemented using the Python\footnote{\url{http://www.python.org/}} language.  The nice features of Python ---such as dynamic typing, extensive numerical libraries, and high programmer productivity--- helped us produce a piece of software which is easy to use and easy to understand.  We are currently using this Python code as a starting point for a parallel version of the code which, in collaboration with members of the developer team, will be incorporated to the PETSc library for scientific computing\cite{petsc-manual}.  This project will be reported elsewhere, but preliminary results are being presented in the upcoming Parallel CFD meeting\cite{CruzBarbaKnepley2008a}.  Our final aim is to contribute to the community of particle simulations with an open source FMM implementation which is parallel and portable.  For the time being, the Python code is being made available publicly and we welcome correspondence from interested researchers\footnote{\url{http://www.maths.bris.ac.uk/~aelab/research/pyFMM.html}}.

Using the Python FMM code, more than 900 calculations were performed, varying the numerical parameters:  $N$, the number of particles, $l$, the number of levels in the tree, and $p$, the truncation level of the multipole expansion.  We looked not only at the maximum error in the domain, which would be the conventional approach;  we also present results showing how the error varies in space, revealing some interesting features of the method.  Through this presentation of the results, we believe a clear characterization of the nature of the FMM approximation is obtained.  

The paper is organized as follows.   The next section presents an outline of the vortex particle method, for completeness.  In \S\ref{fmm}, we offer an overview of the FMM, with some details of our implementation.  Following, in \S\ref{errors}, we discuss briefly the sources of errors in the FMM algorithm.  And finally, \S\ref{results} reports the detailed experiments using the FMM for evaluation of the velocity of $N$ vortex particles;  the behavior of the method will be illustrated for varying parameters, as well as the impact on the efficiency of the calculation, for different problem sizes.  

